Computational Interpretations of Markov's principle

Markov's principle is a statement that originated in the Russian school of Constructive Mathematics and stated originally that "if it is impossible that an algorithm does not terminate, then it will terminate". This principle has been adapted to many different contexts, and in particular we are interested in its most common version for arithmetic, which can be stated as "given a total recursive function f , if it is impossible that there is no n for which f(n) = 0, then there exists an n such that f(n) = 0". This is in general not accepted in constructivism, where stating an existential statement requires one to be able to show at request a witness for the statement: here there is no clear way to choose such an n. We introduce more in detail the context of constructive mathematics from different points of view, and we show how they are related to Markov's principle. In particular, several realizability semantics are presented, which provide interpretations of logical systems by means of different computational concepts (mainly, recursive functions and lambda calculi). This field of research gave origin to the well known paradigm often called Curry-Howrd isomorphism, or also propositions as types, that states a correspondence between proofs in logic and programs in computer science. Thanks to this the field of proof theory, that is the metamathematical investigations of proofs as mathematical objects, became of interest for computer science and in particular for the study of programming languages. By using modern research on the Curry-Howard isomorphism, we will obtain a more refined interpretation of Markov's principle. We will then use this results to investigate the logical properties of systems related to the principle, and introduce a proof transformation technique to interpret constructively some non-constructive proofs of arithmetic.

==> embot.tex <==
\section{Another constructive system based on delimited exceptions}
We have just seen that any proof of a simply existential statement can be adequately modified to only use Markov's principle and no other classical reasoning. Given the constructive properties of Markov's principle, this suggests that proofs of this kind should also allow a direct interpretation in the spirit of the Curry-Howard correspondence (in addition to the one obtained by simply transforming the proofs into proofs using Markov's principle). However as we noted before the \emmeno rule does not lead to a clear computational interpretation. We should then define a new system, and prove its equivalence with $\HA+\EM^-$.

We consider a generalization of the \emeno rule in the form of the \emenne{n} rules, derived naturally from the ones defined in \cite{Aschieri16}:
  \begin{prooftree}
    \AxiomC{$\Gamma, \forall \alpha \emp{} \vdash \exists x C$}
    \AxiomC{$\Gamma, \exists \alpha \emp{}^\bot \vdash \exists x C$}
    \RightLabel{\emeno}
    \BinaryInfC{$\Gamma \vdash \exists x C$}
  \end{prooftree}
  \begin{prooftree}
    \AxiomC{$\Gamma, \forall \alpha A \vdash \exists x C$}
    \AxiomC{$\Gamma, \exists \alpha A^\bot \vdash \exists x C$}
    \RightLabel{\emenne{n}}
    \BinaryInfC{$\Gamma \vdash \exists x C$}
  \end{prooftree}

Where $C$ is quantifier-free, and $A$ is a formula in prenex normal form with $n-1$ alternating quantifiers, the outermost being $\exists$. $A^\bot$ is defined as follows:
\begin{itemize}
\item For atomic predicates $\emp{}$, $\emp{}^\bot$ is the complement of the preidcate $\emp{}$
\item For prenex formulas with alternating quantifiers $A$,  if $A=\mathtt{Q}_{1} \alpha_{1}\,\mathtt{Q}_{2} \alpha_{2}\ldots \mathtt{Q}_{n} \alpha_{n}\, \emp{}$, with $\mathtt{Q}_{i}\in\{\forall,\exists\}$ for $i=1\ldots n$, then $A^{\bot}=\overline{\mathtt{Q}}_{1} \alpha_{1}\,\overline{\mathtt{Q}}_{2} \alpha_{2}\ldots \mathtt{\overline{Q}}_{n} \alpha_{n}\, \emp{}^{\bot}$, where $\mathtt{\overline{Q}}_{i}\in \{\forall,\exists\}\setminus \{\mathtt{Q}_{i}\}$, for $i=1\ldots n$.
\end{itemize}

The system $\HA+\EM^\bot$ is obtained by adding the \emenne{n} rule to $\HA$ for all $n$. The new system is equivalent to the one we studied so far:
\begin{thm}
  $\HA+\EM^\bot \vdash F$ if and only if $\HA+\EM^- \vdash F$
\end{thm}
\begin{proof}
  System $\HA+\EM^\bot$ is at least as strong as $\HA + \EM^-$: since
  it contains the rule \emeno, it can prove Markov's principle; in the
  first section we have seen that the rule \emmeno is equivalent to
  Markov's principle and thus $\HA+\EM^\bot \vdash \textsc{em}^-$ .

  Conversely, it is not stronger than $\HA+\EM^-$. We know that we can
  formalize in the system $\HA + \EM^-$ any classical proof of a
  simply existential statement. It can be easily seen that
  $\forall \alpha A \lor \exists \alpha A^\bot$ is a classical
  tautology, and therefore using an \emenne{n} rule corresponds
  directly to a classical proof making use of the proof of the
  tautology in a disjunction elimination. Therefore any \emenne{n}
  rule can be formalized in $\HA+\EM^-$.
\end{proof}
\subsubsection{Curry-Howard correspondence for $\HA+\EM^\bot$}
In order to provide a proof term for the rule \emuno, we introduced a mechanism of delimited exception handling. How can we generalize this mechanism to the new setting? Clearly, in the case of the rule \emeno in $\HA+\EM^\bot$ we can just reuse the term we introduced in $\HA+\EM_1^-$:


$$\begin{array}{c} \Gamma, a: \forall \alpha\, \emp{} \vdash u: C\ \ \ \ \ \ \ \Gamma, a: \exists \alpha\,\emp{}^\bot \vdash v:C\\
\hline \Gamma\vdash  {u}\, |  |_{a}\,{v} : C
\end{array}\ \textsc{em}^-_1$$

If we proceed in a similar way, we can introduce the term ${u}\, | | |_{a}\,{v}$ to decorate the conclusion of the rule \emenne{2}:
 
$$\begin{array}{c} \Gamma, a: \forall \alpha\,\exists \beta\, \emp{}^\bot \vdash u: C\ \ \ \ \ \ \ \Gamma, a: \exists \alpha\,\forall \beta\,\emp{} \vdash v:
C\\ \hline \Gamma\vdash  {u}\, | | |_{a}\,{v} : C
\end{array}\ \textsc{em}^-_2$$

\begin{figure*}[!htb]

\footnotesize{

\begin{description}

\item[Grammar of Untyped Proof Terms]
\[t,u, v::=\ x\  |\ tu\ |\ tm\ |\ \lambda x\, u\  |\ \lambda \alpha\, u\ |\ \langle t, u\rangle\ |\ u\,\pi_0\ |\ u\,\pi_{1} \ |\ \inj_{0}(u)\ |\ \inj_{1}(u)\  |\ t[x.u, y.v]\ |\ (m,t)\ |\ t[(\alpha, x). u]\]
\[|\ (\Ez{}{u}{v})\ |\ (u\, |\,|\,\ldots |_{a}\,{v})\ |\ \Hypz{a}{\forall \alpha A}\ |\ {\Witz{a}{\exists \alpha A^\bot}}\ \True \ |\ \rec u v m \ |\ \mathsf{r}t_{1}\ldots t_{n}
\]
where $m$ ranges over terms of $\Language$, $x$ over proof-term variables, $\alpha$ over first-order variables, $a$ over hypothesis variables and ${A}$ is a prenex formula with alternating quantifiers and negative propositional matrix or is a simply universal formula.

We assume that in the term ${u}\, |\,|\,\ldots |_{a}\,{v}$, there is some formula $A$, such that $a$ occurs free in $u$ only in subterms of the form $\Hypz{a}{\forall \alpha A}$ and $a$ occurs free in $v$ only in subterms of the form $\Witz{a}{\exists \alpha A^\bot}$, and the occurrences of the variables in $A$ different from $\alpha$ are free in both $u$ and $v$.

\item[Contexts] With $\Gamma$ we denote contexts of the form $e_1:A_1, \ldots, e_n:A_n$, where each $e_{i}$ is either a proof-term variable $x, y, z\ldots$ or an $\EM$ hypothesis variable $a, b, \ldots$, and $e_{i}\neq e_{j}$ for $i\neq j$.

\item[Axioms] %AXIOM
$\begin{array}{c}   \Gamma, x:{A}\vdash x: A
\end{array}\ \ \ \ $
$\begin{array}{c}   \Gamma, a:{\forall {\alpha}\, A}\vdash  \Hypz{a}{\forall \alpha A}:  \forall{\alpha}\, A
\end{array}\ \ \ \ $
$\begin{array}{c}   \Gamma, a:{\exists \alpha\,  A\vdash {\Witz{a}{\exists \alpha A^\bot}}:  \exists{\alpha}\,  A}
\end{array}$\\
%$\begin{array}{c}   \Gamma, a: \prop{P}\vdash  \Hypz{}{\emp{}}:   \emp{}
%\end{array}\ \ \ \ $\\

\item[Conjunction] %CONJUNCTION
$\begin{array}{c}  \Gamma \vdash u:  A\ \ \ \Gamma\vdash t: B\\ \hline \Gamma\vdash \langle
u,t\rangle:
A\wedge B
\end{array}\ \ \ \ $
$\begin{array}{c} \Gamma \vdash u: A\wedge B\\ \hline\Gamma \vdash u\,\pi_0: A
\end{array}\ \ \ \ $
$\begin{array}{c}  \Gamma \vdash u: A\wedge B\\ \hline \Gamma\vdash u\,\pi_1 : B
\end{array}$\\\\


\item[Implication] %IMPLICATION
$\begin{array}{c}  \Gamma\vdash t: A\rightarrow B\ \ \ \Gamma\vdash u:A \\ \hline
\Gamma\vdash tu:B
\end{array}\ \ \ \ $
$\begin{array}{c}  \Gamma, x:A \vdash u: B\\ \hline \Gamma\vdash \lambda x\, u:
A\rightarrow B
\end{array}$\\\\
\item[Disjunction Introduction] %DISJUNCTION
$\begin{array}{c}  \Gamma \vdash u: A\\ \hline \Gamma\vdash \inj_{0}(u): A\vee B
\end{array}\ \ \ \ $
$\begin{array}{c}  \Gamma \vdash u: B\\ \hline \Gamma\vdash\inj_{1}(u): A\vee B
\end{array}$\\\\



\item[Disjunction Elimination] $\begin{array}{c} \Gamma\vdash u: A\vee B\ \ \ \Gamma, x: A \vdash w_1: C\ \ \ \Gamma, y:B\vdash w_2:
C\\ \hline \Gamma\vdash  u\, [x.w_{1}, y.w_{2}]: C
\end{array}$\\\\

\item[Universal Quantification] %FOR ALL
$\begin{array}{c} \Gamma \vdash u:\forall \alpha A\\ \hline  \Gamma\vdash um: A[m/\alpha]
\end{array} $
$\begin{array}{c}  \Gamma \vdash u: A\\ \hline \Gamma\vdash \lambda \alpha\, u:
\forall \alpha A
\end{array}$\\

where $m$ is any term of  the language $\Language$ and $\alpha$ does not occur
free in any formula $B$ occurring in $\Gamma$.\\

\item[Existential Quantification] %EXISTS
$\begin{array}{c}\Gamma\vdash  u: A[m/\alpha]\\ \hline \Gamma\vdash (
m,u):
\exists
\alpha A
\end{array}$ \ \ \ \
$\begin{array}{c} \Gamma\vdash u: \exists \alpha A\ \ \ \Gamma, x: A \vdash t:C\\
\hline
\Gamma\vdash u\, [(\alpha, x). t]: C
\end{array} $\\

where $\alpha$ is not free in $C$
nor in any formula $B$ occurring in $\Gamma$.\\

\item[Induction] %INDUCTION
$\begin{array}{c} \Gamma\vdash u: A(0)\ \ \ \Gamma\vdash v:\forall \alpha^{\Nat}.
A(\alpha)\rightarrow A(\suc(\alpha))\\ \hline \Gamma\vdash\lambda \alpha^{\Nat} \rec uv\alpha :
\forall
\alpha^{\Nat} A
\end{array}$

\item[Post Rules] %ATOMIC RULES
$\begin{array}{c} \Gamma\vdash u_1: A_1\ \Gamma\vdash u_2: A_2\ \cdots \ \Gamma\vdash u_n:
A_n\\ \hline\Gamma\vdash u: A
\end{array}$

where $A_1,A_2,\ldots,A_n,A$ are atomic formulas of $\HA$ and the rule is a Post rule for equality, for a Peano axiom or for a classical propositional
tautology or for booleans and if $n>0$, $u=\mathsf{r} u_{1}\ldots u_{n}$, otherwise $u=\True$.


%\item[$\EM_{0}$]$\begin{array}{c} \Gamma, a:  \emp{}^{\bot} \vdash u: C\ \ \ \ \Gamma, a:  \emp{} \vdash v:
%C\\ \hline \Gamma\vdash  \Ez{}{u}{v} : C 
%\end{array}\ (\prop{P}\mbox{ negative})$ 

\item[$\EM_n^-$]$\begin{array}{c} \Gamma, a: \forall {\alpha}\, A \vdash u: C\ \ \ \ \Gamma, a:  \exists \alpha\, A^{\bot} \vdash v:
C\\ \hline \Gamma\vdash  u\underbrace{|\,|\,\ldots |_{a}}_{n+1 \mbox{{\tiny bars}}}\, v : \mathsf{C}
\end{array}$\\ 

where $\mathsf{C}$ is atomic, $A$ is a formula with alternating quantifiers and: i)  when $n=1$, $A=\prop{P}$ with $\prop{P}$ negative; ii) when $n> 1$, $A=\exists \alpha_{1}\,\forall \alpha_{2}\exists \alpha_{3}\ldots\mathtt{Q}_{n-1} \alpha_{n-1}\, \prop{P}$, with $\prop{P}$ negative and $\mathtt{Q}_{n-1}\in\{\forall,\exists\}$.\\\\

\end{description}
}
\caption{Term Assignment Rules for $\HA+\EM^\bot$}\label{fig:system}
\end{figure*}


The complete term system together with the type assignment is described in \cref{fig:system}
But how can we use this term? Remaining faithful to the ideas of \emph{learning}, assume we start by reducing inside $u$ in order to get a proof of $C$; when in such reduction we need to use an instance $\exists \beta \emp{}^\bot[\alpha/m]$ of the universal assumption on a closed first order term $m$, we do not have a direct way to check its truth: therefore an exception is automatically thrown, which results in the creation of a duplicated environment. In one environment, we assume that the instance holds; therefore, we have \emph{learned} new information: we erase from $u$ the premise $\forall \alpha\,\exists \beta\,\emp{}^\bot$ of all eliminations of $\forall \alpha\,\exists\beta\, \emp{}^\bot$ having as conclusion $\exists\beta\,\emp{}^\bot[m/\alpha]$ and obtain the term $u^-$. In the other environment, we assume that it doesn't: here we have a much bigger progress, since we know that $\forall \beta \emp{}[m/\alpha]$. We obtain $v^{+}$ by replacing all occurrences of the hypothesis $\exists \alpha\,\forall\beta\,\emp{}$ with a proof of it by an introduction rule with premise $\forall\beta\,\emp{}[m/\alpha]$. We can see that the two assumptions are now of a lower complexity: the two environments can be put in communication using the rule \emuno. Therefore the application of \emenne{2} can be reduced to

\begin{prooftree}

\AxiomC{$\Gamma,  b:\forall \beta\, \emp{}[m/\alpha] \vdash v^{+}: C\qquad$}

\AxiomC{$\Gamma, a: \forall \alpha\,\exists \beta\, \lnot\emp{}, b:\exists\beta\, \lnot\emp{}[m/\alpha]\vdash  u^{-}: C$}
\AxiomC{$\Gamma, a: \exists \alpha\,\forall \beta\,\emp{}\vdash v: C$}
\RightLabel{\emenne{2}}
\insertBetweenHyps{\hskip 8pt}
\BinaryInfC{$\Gamma,  b: \exists \beta\,\lnot\emp{}[m/\alpha]\vdash {u^{-}}\, | | |_{a}\,{v}: C$}
\RightLabel{\emenne{1}}
\insertBetweenHyps{\hskip -19pt}
\BinaryInfC{$\Gamma\vdash \E{b}{v^{+}}{({u^{-}}\, | | |_{a}\, {v})}: C$}
\end{prooftree}

The two environments are parallel, but can still communicate with each other: an exception may at any moment be raised by $v^{+}$ and a term be passed in particular to $u^{-}$. The reduction rules for all the \emenne{n} rules are just the generalization of this reduction.

In order to implement the reduction rules, we will need to introduce new terms associated to the assumptions. In a totally similar way as before, we have

%\[\hyp{a}{\alpha}{A}\]
%\[\wit{a}{\alpha}{A^{\bot}}\]

$$\begin{array}{c}   \Gamma, a: \forall \alpha\, A \vdash   \Hypz{a}{\forall \alpha A} :  \forall \alpha\, A
\end{array}\ \ \ \
\begin{array}{c}   \Gamma, a:{\exists \alpha\, A^{\bot}}\vdash \Witz{a}{\exists \alpha A^\bot}:  \exists\alpha\, A^{\bot}
\end{array}$$

where the first term introduces an hypothesis, the second waits for a witness (again, they can be thought in correspondence with \texttt{raise} and \texttt{catch}) and $a$ represents a communication channel. However, there is a major difference with the system of the previous chapter: as we said, an exception is now automatically raised whenever the term $\Hypz{a}{\forall \alpha A}$ is used, since we cannot check its truth; the ordinary computation might continue, and raise multiple exceptions. The computation is aborted only in the case of an exception relative to an atomic formula, when we can finally check the value of the term.

Before defining the reduction rules, we should define a new exception substitution, replacing the old witness substitution
\begin{definition}[Exception Substitution]\label{def:witsub}
\label{definition-witsub} Suppose $v$ is any proof term and $e=(m,b)$, where $m$ is a  term of $\Language$ and $\mathsf{b}$ an $\EM$-hypothesis variable $b$. Then:
\begin{enumerate}
%% La sostituzione senza comunicazione non dovrebbe più servire
%\item If $\mathsf{b}=\epsilon$ and every free occurrence of $a$ in $v$ is of the form $\Witz{a}{\exists \alpha \prop{P}}{}$, we define $$v[a:=e]$$ as the term obtained from $v$ by replacing each subterm $\wit{a}{\alpha}{P}$ corresponding to a free occurrence of $a$ in $v$ by $(m, \True)$.%,
%\item If $\mathsf{b}=\epsilon$ and every free occurrence of $a$ in $v$ is of the form $\hyp{a}{\alpha}{P}$, we define $$v[a:=e]$$ as the term obtained from $v$ by replacing  each subterm $\hyp{a}{\alpha}{P}m$ corresponding to a free occurrence of $a$ in $v$ by $\Hypz{}{\prop{P}[m/\alpha]}$.
 \item If every free occurrence of $a$ in $v$ is of the form $\hyp{a}{\alpha}{A}$, and $\forall \alpha\, A$ is prenex with alternating quantifiers with $A$ non propositional, we define $$v[a:=e]$$ as the term obtained from $v$ by replacing, without capture of $b$,  each subterm $\Hypz{a}{\forall \alpha A}m$ corresponding to a free occurrence of $a$ in $v$ by $ \Witz{b}{A[m/\alpha]}$.

\item If every free occurrence of $a$ in $v$ is of the form $\Witz{a}{\exists \alpha A}{}$, and $\exists \alpha\, A$ is prenex with alternating quantifiers with $A$ non propositional, we define $$v[a:=e]$$ as the term obtained from $v$ by replacing, without capture of $b$,  each subterm $\Witz{a}{\exists \alpha A}$ corresponding to a free occurrence of $a$ in $v$ by $(m, \Hypz{b}{A[m/\alpha]})$.%, if $A$ is not propositional, by $(m, \Hypz{}{A[m/\alpha]})$ otherwise.

\item If every free occurrence of $a$ in $v$ is of the form $\Witz{a}{\exists \alpha \mathsf{P^\bot}}{}$, and $\emp{}^\bot$ is atomic, we define $$v[a:=e]$$ as the term obtained from $v$ by replacing, replacing every occurrence of $\wit{a}{\alpha}{P}$ in $v$ by $(n,\True)$ if $\emp{}[n/\alpha] \equiv \False$, and by $(n,\hyp{a}{\alpha}{\alpha=0}\suc 0)$ otherwise.
 \end{enumerate}
 \end{definition}

We can now describe the reduction rules (\cref{fig:red})

\begin{figure*}[!htb]
\footnotesize{
\begin{description}

\item[Reduction Rules for $\HA$] 
\[(\lambda x. u)t\mapsto u[t/x]\qquad (\lambda \alpha. u)t\mapsto u[t/\alpha]\]
\[ \pi_{i}\pair{u_0}{u_1}\mapsto u_i, \mbox{ for i=0,1}\]
\[\inj_{i}(u)[x_{1}.t_{1}, x_{2}.t_{2}]\mapsto t_{i}[u/x_{i}], \mbox{ for i=0,1} \]
\[(n, u)[(\alpha,x).v]\mapsto v[n/\alpha][u/x], \mbox{ for each numeral $n$} \]
\[\rec u v 0 \mapsto u\]
\[\rec u v (\suc n) \mapsto v n (\rec u v n), \mbox{ for each numeral $n$} \]

\item[Permutation Rules for $\EM_{n}$]
\[(\Ecrom{a}{u}{v}) w \mapsto \Ecrom{a}{uw}{vw},\mbox{ if $a$ does not occur free in $w$} \]
\[(\Ecrom{a}{u}{v})\pi_{i}  \mapsto \Ecrom{a}{u\pi_{i}}{v\pi_{i}} \]
\[(\Ecrom{a}{u}{v})[x.w_{1}, y.w_{2}] \mapsto \Ecrom{a}{u[x.w_{1}, y.w_{2}]}{v[x.w_{1}, y.w_{2}]},\mbox{ if $a$ does not occur free in $w_{1},w_{2}$}
\]
\[(\Ecrom{a}{u}{v})[(\alpha, x).w] \mapsto \Ecrom{a}{u[(\alpha, x).w]}{v[(\alpha, x).w]}, \mbox{ if $a$ does not occur free in $w_{1},w_{2}$}
\]

\item[Reduction Rules for $\EM_1$]
\[\E{a} u v\mapsto u,\ \mbox{ if $a$ does not occur free in $u$ }\]
\[\E{a} u v\mapsto v[a:=n],\ \mbox{ if $\hyp{a}{\alpha}{P}n$ occurs in $u$ and $\emp{} [n/\alpha]$ is closed and $\emp{} [n/\alpha]=\False$ }\]
\[(\hyp{a}{\alpha}{P})n \mapsto \True \mbox{ if $\emp{}[n/\alpha]$ is \emph{closed} and $\emp{}[n/\alpha] \equiv \True$}\] 
% \[[a]\wit m \mapsto (n, \True) \mbox{ for each numeral $n$ }\]


\item[Reduction Rules for $\EM_{n}$ (n > 1)]
\[\Hyp{a}{A}{\alpha}m \mapsto \Witz{b}{A[m/\alpha]}, \mbox{ $b$ fresh}\]
\[\Ecrom{a}{u}{v}\mapsto u,\ \mbox{ if $a$ does not occur free in $u$ }\]

\[\Esucc{a}{u}{v}\mapsto \Ecrom{\mathsf{b}}{v[a:=e]}{(\Esucc{a}{u[a:=e]}{v})}
%\comment{\overset{def}{=}v[(n,\True)/\Wit{a}{\emp{}}{{\alpha}}]}
,\mbox{ whenever $u$ has some \emph{active} subterm $\Hyp{a}{A}{\alpha}m$, $e=(m,b)$ and}\]
\[\mbox{$b$ is a fresh $\EM_{}$-hypothesis variable $b$ }\]
%for $u$ and $v$.
\end{description}}
\caption{Reduction Rules for $\HA$ + $\EM^\bot$}\label{fig:red}
\end{figure*}
%% TODO: constructivity
\begin{proposition}[Normal Form Property]\label{prop:pnf}
Let $\prop{P}, \prop{P}_{1}, \ldots, \prop{P}_{n}$ be negative propositional formulas. Suppose that 
$$\Gamma=x_1: \prop{P}_{1},\ldots,x_n: \prop{P}_{n},  a_{1}: \forall {\alpha}_{1}{A}_{1},\ldots, a_{m}:\forall {\alpha}_{m}{A}_{m}, $$ 
and  $\Gamma\vdash t:\exists {\alpha}\, \prop{P}$ or $\Gamma\vdash t: \prop{P}$, with $t\in\nf$ and having all its free variables among $x_{1}, \ldots, x_{n}, a_{1}, \ldots, a_{m}$. Then:\\
\begin{enumerate}

\item Either every occurrence in $t$ of every  term  $\Hyp{a_{i}}{{A_i}}{{\alpha_{i}}}$ is of the active form $\Hyp{a_{i}}{{A_i}}{{\alpha_{i}}}m$, where $m$ is a  term of $\Language$; or $t$ has an active subterm of the form $\Hyp{a_{i}}{{A_i}}{{\alpha_{i}}}m$, for some non simply universal formula $A_i$ and term  $m$  of $\Language$. \\

\item Either  $t=(m, u)$ or $t=\lambda x\, u$ or $t=\langle u, v \rangle$ or $t=\Ez{}{u}{v}$ or $t=\Ecrom{a}{u}{v}$ or $t=\Hypz{}{\prop{P}}$ or $t=x_{i}\, t_{1}\, t_{2}\ldots t_{n} $ or $t=\Hyp{a_{i}}{{A}_{i}}{{\alpha}}m\, t_{2}\ldots t_{n}$.
 \end{enumerate} 

\end{proposition}

\begin{proof} 
We prove 1. and 2. simultaneously and by induction on  $t$. There are several cases, according to the shape of $t$:\\
\begin{itemize}
\item $t=(m, u)$, $\Gamma\vdash t:\exists {\alpha}\, \prop{P}$ and $\Gamma \vdash u: \prop{P}[m/\alpha]$. We immediately get 1. by induction hypothesis applied to $u$, while  2. is obviously verified.\\

\item $t=\lambda x\, u$, $\Gamma \vdash t: \prop{P}=\prop{Q}\rightarrow \prop{R}$ and $\Gamma, x: \prop{Q} \vdash u: \prop{R}$. We immediately get 1. by induction hypothesis applied to $u$, while  2. is obviously verified.\\

\item $t=\langle u, v\rangle$, $\Gamma \vdash t: \prop{P}=\prop{Q}\land \prop{R}$, $\Gamma \vdash u: \prop{Q}$ and $\Gamma \vdash v: \prop{R}$. We immediately get 1. by induction hypothesis applied to $u$, while  2. is obviously verified.\\

\item $t=\Ez{}{u}{v}$, $\Gamma, a: \prop{Q}^{\bot} \vdash u: \exists {\alpha}\, \prop{P}$ (resp. $u: \prop{P}$) and $\Gamma, a: \prop{Q} \vdash v: \exists {\alpha}\,\prop{P}$ (resp. $v: \prop{P}$). We immediately get the thesis by induction hypothesis applied to $u$ and $v$, while 2. is obviously verified.\\

\item  $t=\Ecrom{a}{u}{v}$, $\Gamma, a: \forall \beta\, A \vdash u: \exists {\alpha}\, \prop{P}$ (resp. $u: \prop{P}$) and $\Gamma, a: \exists {\beta}\, A^{\bot}\vdash v: \exists {\alpha}\,\prop{P}$ (resp. $v: \prop{P}$).  We first observe that $a$ must occur free in $u$: otherwise,  $t=\Ecrom{a}{u}{v}\mapsto u$, which would yield a contradiction to $t\in \nf$. Now, by induction hypothesis, 1. holds with respect to $u$. Moreover, it cannot be that every occurrence in $u$ of every  hypothesis variable $a_{i}$ or $a$ corresponds to an active term: otherwise, in particular, $u$ would have an active subterm of the form $\Hyp{a}{A}{\beta}m$, for some $m\in\Language$, and  thus
$t=\Esucc{a}{u}{v}\mapsto \Ecrom{\mathsf{b}}{v[a:=e]}{(\Esucc{a}{u[a:=e]}{v})}$, with $e=(m,\mathsf{b})$: but  $t\in\nf$. Therefore, $u$ has an active subterm of the form $\Hyp{a_{i}}{{A_i}}{{\alpha_{i}}}m$, for some non simply universal formula $A_i$  and  $m\in\Language$. We have thus established 1. for $t$, while 2. is obviously verified. 
\\

\item $t=\Hyp{a_{i}}{A_{i}}{{\alpha}}$. This case is not possible, for  $\Gamma\vdash t:\exists {\alpha}\, \prop{P}$ or $\Gamma\vdash t: \prop{P}$.   \\

\item $t=\Hypz{}{\prop{P}}$. In this case, 1. and 2. are trivially true. \\

\item $t$ is obtained by an elimination rule and we can write it as $r\, t_{1}\,t_{2}\ldots t_n$ where $r$ is not an application (this notation has been explained in Section~\ref{section-system}). Notice that in this case $r$ cannot be a redex neither a term of the form $\Ecrom{a}{u}{v}$ nor $\Ez{}{u}{v}$ because of the permutation rules and  $t\in \nf$.
%Then, if we denote for a moment the terms of the form $\pi_{i} u$ as $u\, \pi_{i}$, we can write $t$, with this notation, as $r \, t_{1}\, t_{2}\ldots t_{n}$ ($n>0$), where $r$ is either a variable $x_{i}$ or a term $\Hyp{a_{i}}{\prop{P}_{i}}{{\alpha}}$ or $\Hypz{}{\prop{P}}$ (it cannot be a redex neither a term of the form $\Ecrom{a}{u}{v}$ nor $\Ez{}{u}{v}$ because of the permutation rules and  $t\in \nf$), and each $t_{i}$ is either a term (when $r \, t_{1}\, \ldots t_{i}$ is obtained by an $\rightarrow$-elimination rule or by a $\forall$-elimination rule) or a constant $\pi_{i}$ (when $r \, t_{1}\, \ldots t_{i}$ is obtained by an $\land$-elimination rule) or an expression $[x_{0}.u_{0}, x_{1}.u_{1}]$ (when $r \, t_{1}\, \ldots t_{i}$ is obtained by an $\lor$-elimination rule) or an expression $[(\alpha, x).u]$ (when $r \, t_{1}\, \ldots t_{i}$ is obtained by an $\exists$-elimination rule). 
We have now two cases:\\
\begin{enumerate}
\item
$r=x_{i}$ (resp. $r=\Hypz{}{\prop{P}}$). Then, since $\Gamma \vdash x_{i}: \prop{P}_{i}$ (resp. $\Gamma \vdash \Hypz{}{\prop{P}}: \prop{P}$), we have that for each $i$, either $t_{i}$  is $\pi_{j}$ or $\Gamma\vdash t_{i}: \prop{Q}$, where $\prop{Q}$ is a propositional formula. By induction hypothesis, each $t_{i}$ satisfies 1. and thus also $t$. 2. is obviously verified. \\

\item  $r=\Hyp{a_{i}}{{A}_{i}}{{\alpha_i}}$. Then, $t_{1}$ is $m$, for some closed term of $\Language$. If $A_{i}$ is not simply universal, we obtain that $t$ satisfies 1., for $t=\Hyp{a_{i}}{{A}_{i}}{{\alpha_i}}m\, t_{2}\ldots t_{n}$. If $A_{i}=\forall\gamma_1\ldots\gamma_k$ $\prop{Q}$, with $\prop{Q}$ propositional, we have that for each $i$, either $t_i$ is a closed term $m_i$ of $\Language$ or  $t_{i}$  is $\pi_{j}$ or $\Gamma\vdash t_{i}: \prop{R}$, where $\prop{R}$ is a propositional formula. By induction hypothesis, each $t_{i}$ satisfies 1. and thus also $t$. 2. is obviously verified.
\end{enumerate}


\end{itemize}


\end{proof}

\begin{definition}[Herbrand Normal Forms] \label{definition-hnf}
We define by induction a set of proof terms, called \emph{Herbrand normal forms}, as follows:
\begin{itemize}
\item Every normal proof-term $(m,u)$ is an Herbrand normal form;
\item if $u$ and $v$ are Herbrand normal forms, $\Ez{}{u}{v}$ is an Herbrand normal form.
\end{itemize}
\end{definition}


\begin{thm}[Herbrand Disjunction Extraction]\label{theorem-extraction}
Let $\exists\alpha\,\prop{P}$ be any closed formula where $\prop{P}$ is atomic. Suppose $\Gamma \vdash t:  \exists \alpha\, \prop{P}$, $t$ is quasi-closed and $t\mapsto^{*} t'\in\nf$. Then $\Gamma \vdash t': \exists \alpha\, \prop{P}$ and $t'$ is an Herbrand normal form   
$$\Ez{}{\Ez{}{\Ez{}{(m_{0}, u_{0})}{(m_{1}, u_{1})}}{}\ldots}{(m_{k}, u_{k})}$$
Moreover, $\Gamma \vdash \prop{P}[m_{1}/\alpha]\lor \dots \lor \prop{P}[m_{k}/\alpha]$.

\end{thm}

\begin{proof}\mbox{} We proceed by induction on $t'$. By the Subject Reduction Theorem \ref{subjectred}, $t': \exists \alpha\, \prop{P}$.  By Proposition \ref{prop:pnf}, $t'$ can only have three possible shapes: 
\begin{enumerate}
\item $t'=\Ecrom{a}{u}{v}$. We show that this cannot happen.  First, $a$ must occur free in $u$, otherwise $t'\notin\nf$. By Proposition \ref{prop:pnf},  we have two possibilities. i) Every  occurrence in $u$ of every  term  $\Hyp{a_{i}}{{A_i}}{{\alpha_{i}}}$, with $a_{i}$ free, is of the active form $\Hyp{a_{i}}{{A_i}}{{\alpha_{i}}}m$, where $m\in\Language$;  in particular this is true when $a_{i}=a$, which implies $t'\notin\nf$. ii) $u$ has an active subterm of the form $\Hyp{a_{i}}{{A_i}}{{\alpha_{i}}}m$, for some non simply universal formula $A_i$ and  $m\in\Language$: since $t'$ is quasi-closed, $a_{i}=a$,  which again implies $t'\notin\nf$. In any case, we have a contradiction. 

\item  $t'=\Ez{}{u}{v}$; then, by induction hypothesis, $u, v$ are Herbrand normal forms, and thus by definition \ref{definition-hnf}, $t'$ is an Herbrand normal form as well.
\item $t'=(m, u)$; then, we are done.

 \end{enumerate}
 We have thus shown that $t'$ is an Herbrand normal form $$\Ez{}{\Ez{}{\Ez{}{(m_{0}, u_{0})}{(m_{1}, u_{1})}}{}\ldots}{(m_{k}, u_{k})}$$ 
 Finally, we have that for each $i$, $\Gamma_{i}\vdash u_{i}: \prop{P}[m_{i}/\alpha]$, for the very same  $\Gamma_{i}$ that types $(m_{i}, u_{i})$ of type $\exists \alpha\, \prop{P}$ in $t'$. Therefore, for each $i$, $\Gamma_{i}\vdash u_{i}^{+}: \prop{P}[m_{1}/\alpha]\lor \dots \lor \prop{P}[m_{k}/\alpha]$, where $u_{i}^{+}$ is of the form $\inj_{i_{1}}(\ldots \inj_{i_{k}}(u_{i})\ldots )$.  We conclude that 
 $$\Gamma \vdash \Ez{}{\Ez{}{\Ez{}{u_{0}^{+}}{u_{1}^{+}}}{}\ldots}{u_{k}^{+}}: \prop{P}[m_{1}/\alpha]\lor \dots \lor \prop{P}[m_{k}/\alpha]$$ 
  \end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "tesi.tex"
%%% End:

